Gradient Clock Synchronization using Reference Broadcasts

In this paper we suggest a method by which reference broadcast synchronization (RBS), and other methods of estimating clock values, can be incorporated in standard clock synchronization algorithms to improve synchronization quality. We advocate a logical separation of the task of estimating the clock values of other nodes in the network from the task of using these estimates to output a logical clock value. The separation is achieved by means of a virtual estimate graph, overlaid on top of the real network graph, which represents the information various nodes can obtain about each other. RBS estimates are represented in the estimate graph as edges between nodes at distance 2 from each other in the original network graph. A clock synchronization algorithm then operates on the estimate graph as though it were the original network. To illustrate the merits of this approach, we modify a recent optimal gradient clock synchronization algorithm to work in this setting. The modified algorithm transparently takes advantage of RBS estimates and any other means by which nodes can estimate each others' clock values.

==> intro.tex <==
\section{Introduction}
%The problem of time synchronization has received renewed attention in the research community in recent years, as 
The evolving field of wireless networks poses new and interesting
challenges to time synchronization, leading to renewed attention to
this venerable problem in recent years. Sensor networks in particular
are subject to constraints on computation power and energy
consumption, and often require a greater degree of synchronization
than traditional distributed applications.

In a multi-hop sensor network it is frequently the case that
neighboring nodes must be closely synchronized, while far-apart nodes
can tolerate greater clock skew: neighboring nodes interfere with each
other when they try to transmit, and are also more likely to cooperate
for the purpose of some local computation. This gives rise to the
problem of \emph{gradient clock synchronization}, in which the
synchronization between two nodes improves the closer they are to each other.
The problem was first formulated
in~\cite{fanlowerbound}, where it is shown that in a network of
diameter $D$, no algorithm can guarantee a skew that is
better than $\Omega(\log D / \log \log D)$ even
between adjacent nodes. Subsequent work has improved the lower bound
to $\Omega(\log D)$, and come up with algorithms that match
it \cite{lenzen08,locher09podc}.

%As well as these challenges,
The wireless broadcast medium also offers opportunities for better synchronization. Although contention may cause unpredictable delays before a message is broadcast, once a message is transmitted, it is received by all nodes in the sender's neighborhood almost instantaneously. Reference broadcast synchronization (RBS) \cite{rbs} takes advantage of this to let the \emph{neighbors} of the sender estimate each other's clock values with great accuracy. RBS can be extended to multi-hop networks, to allow any node in the network to estimate the clock value of any other node. However, by itself, RBS does not output a \emph{logical clock} at every node, and so it is not a clock synchronization algorithm in the traditional sense.

In this paper we suggest an approach by which RBS, or any other estimation method (including external time sources), can be seamlessly incorporated in many clock synchronization algorithms, in order to reduce the effective diameter of the network and achieve better synchronization. We suggest a separation between the \emph{estimate layer}, which is responsible for estimating other nodes' clock values, and the algorithm that uses these estimates to compute a local logical clock.
%at every node.
The estimate layer runs underneath the %clock synchronization
algorithm and provides it with an \emph{estimate graph} $\Gest$. Each edge $\set{u,v}$ of $\Gest$ represents an estimate that node $u$ can get for node $v$'s clock value (and vice-versa), along with an associated \emph{uncertainty}. RBS estimates are represented in $\Gest$ as edges between nodes at distance 2 from each other in the original network graph.

Almost any clock synchronization algorithm can be used on top of the estimate layer, as long as the algorithm can handle
%heterogeneous networks in which the uncertainty varies from link to link.
networks with non-uniform uncertainty on the links.
%In the resulting framework,
The resulting synchronization between %two
nodes $u,v$ depends on their \emph{effective distance} $\dist(u,v)$, and on the \emph{effective diameter} of the network graph. These are defined by the corresponding distances in the estimate graph $\Gest$. Using RBS it is possible to reduce the effective diameter to $O( (\drift\cdot\delay + \ru) \cdot D + \delay)$, where $D$ is the diameter of the original network, $\delay$ is a bound on the message delay, $\drift$ is a bound on clock drift (typically very small), and $\ru$ is a bound on the receiver uncertainty (also very small \cite{rbs}), which bounds the time it takes a node to process a message it receives.

Our main contributions are as follows. In Section~\ref{sec:est} we
define the estimate layer, and show how to incorporate point-to-point
messages and RBS. In Section~\ref{sec:alg}, we illustrate the
applicability of our approach by modifying the algorithm
of~\cite{locher09podc} to work on top of the estimate layer.
Significantly, this involves extending it to a heterogeneous network;
in~\cite{locher09podc} it is assumed that all links are subject to the
same bounds on message delay. Finally, in Section~\ref{sec:analysis}
we prove that the algorithm achieves gradient clock synchronization,
with the skew between nodes $u$ and $v$ bounded by
$O(\dist(u,v)\cdot\log_{1/\drift} D)$ in networks with
effective diameter $D$ and drift bounded by $\drift$. This
is asymptotically optimal. The proof is based on the proof
in~\cite{locher09podc}, but in our view it is cleaner and somewhat
simpler.

In a companion paper to this one \cite{spaa09}, we consider
the problem of gradient clock synchronization in \emph{dynamic}
networks, and show that the weighted-graph approach employed here is
useful in that context as well.

%We believe that the improved proof presented in
%Section~\ref{sec:analysis} is helpful in understanding the original
%algorithm of~\cite{locher09podc} as well as the modified version
%presented here. This is significant because to our knowledge, this is
%the only optimal gradient clock synchronization algorithm currently
%known. In addition, in a companion paper to this one \cite{spaa09}, we
%consider the problem of gradient clock synchronization in
%\emph{dynamic} networks, and show that the weighted-graph approach
%employed here is useful in that context as well. In the future we
%intend to adapt the algorithm further to work in the dynamic setting.


==> relatedwork.tex <==

\section{Related Work}
\label{sec:relatedwork}

The problem of establishing a common notion of time is at the core of
many distributed systems and applications and has thus been widely
studied, both from a theoretical and a practical point of view. In
most of the existing work on clock synchronization, the nodes of a
network compute estimates about each others' clock values by exchanging
messages. Based on the obtained information, each node computes a
local logical clock. Typically, the accuracy of clock estimates is
determined by the uncertainty about the propagation delay of messages.
In \cite{lundelius84}, it is shown that even if hardware clocks
experience no drift, no clock synchronization algorithm can prevent a
clock skew of $\Omega(D)$ in a network of diameter $D$. This lower
bound on the maximum clock skew between any two nodes is matched by an
algorithm described in \cite{srikanth87} and by many subsequent
algorithms (e.g.\
\cite{attiya96,fanalgorithm,locher09podc,lenzen08,ostrovsky99,patt-shamir94}).
Clock synchronization algorithms and lower bounds that %make use of
accommodate
non-uniform propagation delays are described, for example, in
\cite{attiya05,cristian89,halpern85}.

In \cite{fanlowerbound}, Fan and Lynch introduced the gradient clock
synchronization problem. It is shown that even on a path of length
$D$, no algorithm can guarantee a clock skew smaller than $\Omega(\log
D/\log\log D)$ between adjacent nodes. This bound has been improved to
$\Omega(\log D)$ in \cite{locher09podc} and it is shown in
\cite{lenzen08,locher09podc} that the new bound in indeed tight.

%\clearpage

The special properties, constraints, and requirements of wireless ad
hoc and sensor networks make clock synchronization especially
challenging. There is a considerable amount of work on the problem
(e.g.\ \cite{fanalgorithm,roemer,sivrikaya,sundararaman}).
Particularly interesting is the work on reference broadcast
synchronization \cite{rbs,karp04}, which exploits the property of
sharing a single communication channel to obtain high accuracy clock
estimates of nearby nodes. 

